Chandra and XMM-Newton Observations of the Bimodal Planck SZ-detected Cluster PLCKG345.40-39.34 (A3716) with High and Low Entropy Subcluster Cores

We present results from Chandra, XMM-Newton, and ROSAT observations of the Planck SZ-detected cluster A3716 (PLCKG345.40-39.34 - G345). We show that G345 is, in fact, two subclusters separated on the sky by 400 kpc. We measure the subclusters' gas temperatures (~ 2-3 keV), total (~ 1-2 x 10^14 solar masses) and gas (~ 1-2 x 10^13 solar masses) masses, gas mass fraction within r500, entropy profiles, and X-ray luminosities (~ 10^43 erg/s). Using the gas density and temperature profiles for both subclusters, we show that there is good (0.8 sigma) agreement between the expected Sunyaev-Zel'dovich signal predicted from the X-ray data and that measured from the Planck mission, and better agreement within 0.6 sigma when we re-computed the Planck value assuming a two component cluster model, with relative amplitudes fixed based on the X-ray data. Dynamical analysis shows that the two galaxy subclusters are very likely (> 97% probability) gravitationally bound, and in the most likely scenario, the subclusters will undergo core passage in 500 +- 200 Myr. The northern subcluster is centrally peaked and has a low entropy core, while the southern subcluster has a high central entropy. The high central entropy in the southern subcluster can be explained either by the mergers of several groups, as suggested by the presence of five giant ellipticals or by AGN energy injection, as suggested by the presence of a strong radio source in one of its massive elliptical galaxies, or by a combination of both processes.

==> Makefile <==
# Format a latex file as DVI, PS or PDF
LATEX := latex
BIBTEX := bibtex
DVIPS := dvips
PS2PDF := ps2pdf
FORMAT := letter

# Root names for bibtex sources
bibroot := $(basename $(wildcard *.bib))

ALL: G345.pdf


.SUFFIXES:
.SUFFIXES: .tex .bib .bbl .dvi .ps

.PRECIOUS: %.bbl %.dvi %.ps

# Zap the implicit rule
%.dvi: %.tex


# Pattern rules
%.pdf: %.ps
	$(PS2PDF) $<

%.ps: %.dvi
	$(DVIPS) -Ppdf -G0 -t $(FORMAT) $* -o

%.dvi: %.tex
	while ( \
	  $(LATEX) $* ; \
	  grep -q "Rerun to get \(citations correct\|cross-references right\)" $*.log ) do true ; \
	done

%.bbl: %.tex %.bib
	$(LATEX) $*
	$(BIBTEX) $*


# For latex sources using bibtex
$(addsuffix .dvi,$(bibroot)): %.dvi: %.bbl


clean:
	rm -f *.dvi *.aux *. *.blg *.log *~

vclean: clean
	rm -f *.ps *.bbl

vvclean: vclean
	rm -f *.pdf


==> pubs-journals.tex <==
% Journal name macros

%% \newcommand\mnras{MNRAS}
%% \newcommand\apj{ApJ}
%% \newcommand\apjl{ApJ}
%% \newcommand\apjs{ApJS}
%% \newcommand\nat{Nature}
%% \newcommand\aap{A\&A}
%% \newcommand\aapr{A\&A}
%% \newcommand\araa{ARAA}
%% \newcommand\physrep{PhysRep}
%% \newcommand\aj{AJ}
%% \newcommand\sovast{SovAst}

%%\newcommand\jcap{J.\ Cosmol.\ Astropart.\ Phys.}

